Neural-based Video Compression on Solar Dynamics Observatory Images

NASA's Solar Dynamics Observatory (SDO) mission collects extensive data to monitor the Sun's daily activity. In the realm of space mission design, data compression plays a crucial role in addressing the challenges posed by limited telemetry rates. The primary objective of data compression is to facilitate efficient data management and transmission to work within the constrained bandwidth, thereby ensuring that essential information is captured while optimizing the utilization of available resources. This paper introduces a neural video compression technique that achieves a high compression ratio for the SDO's image data collection. The proposed approach focuses on leveraging both temporal and spatial redundancies in the data, leading to a more efficient compression. In this work, we introduce an architecture based on the Transformer model, which is specifically designed to capture both local and global information from input images in an effective and efficient manner. Additionally, our network is equipped with an entropy model that can accurately model the probability distribution of the latent representations and improves the speed of the entropy decoding step. The entropy model leverages a channel-dependent approach and utilizes checkerboard-shaped local and global spatial contexts. By combining the Transformer-based video compression network with our entropy model, the proposed compression algorithm demonstrates superior performance over traditional video codecs like H.264 and H.265, as confirmed by our experimental results.

==> ACWE.tex <==
% This section can be added to a project using the command \input{ACWE} This section relies on the figures in the \fig\ACWE folder, and the citations added to the .bib file that are marked "% Added for ACWE"

\subsection{Example of the Impact on Downstream Use Applications} \label{sec:experiments:ACWE}

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figs/ACWE/ACWEresize_param1.aia.lev1_euv_12s.2010-09-18T000008Z.193.image_lev1.fits.Compare.png}
    \caption{Effects of proposed compression scheme on CH detection via ACWE. The top left image is the original solar EUV image. At this wavelength CHs appear as dark regions. The CH segmentation on the original image is in the top right. The remaining images are comparisons of the original ACWE segmentation with the segmentation generated from the compressed image. In each image purple regions were only identified as CHs in the original segmentation, yellow regions were identified as belonging to a CH only in the compressed image segmentation, green regions were identified as CHs in both segmentations, and blue regions were not identified as CHs in either segmentation.}
    \label{fig:ACWEneuralExample}
\end{figure*}

In order to provide an example of the effects of the proposed compression scheme on data science applications, the coronal hole (CH) detection and segmentation scheme outlined in \cite{boucheron2016segmentation}, which is an extension of the active contours without edges (ACWE) algorithm of \cite{chan2001}, was applied to four 193~{\AA} Solar EUV images. The effects of compression were determined by comparing the similarity of the resulting CH regions at various bit rates to the CH regions identified on the original Level 1 193~{\AA} EUV images. 

CHs are regions of low-density, low-temperature plasma within the Sun's corona. These regions are associated with open magnetic field lines, and are sources of high-speed solar wind \cite{Altschuler1972,Munro1972,Wang1990,Wang1996}. For this reason, accurate delineation of CH boundaries and extents is important for accurate space weather modeling and prediction \cite{Wang1990,Arge2003,Arge2004}. The segmentation scheme outlined in \cite{boucheron2016segmentation} combines threshold-based detection, which is a common method of detecting CHs \cite{Reiss2021}, with a region refinement algorithm that further refines the initial segmentation based on the homogeneity of the region. By using the algorithm of \cite{boucheron2016segmentation} we can verify that region intensity and underlying structure necessary for accurate delineation of coronal holes are both preserved in the compressed images.

ACWE is an iterative process wherein an initial contour or ‘seed’ is manipulated on a pixel-by-pixel basis across multiple iterations in order to minimize an energy functional. The ACWE energy functional is minimized by balancing three forces which seek to 1: minimize the length of the contour, 2: maximize the homogeneity of the foreground (or CH region), and 3: maximize the homogeneity of the background or non-CH region \cite{chan2001}. Each force is subject to a user-defined weight which defines the relative importance of achieving each goal \cite{chan2001}. Unlike the process outlined in \cite{boucheron2016segmentation}, ACWE was performed on the images at the original resolution of $4096\times4096$ pixels. The rest of the process follows the method outlined in \cite{boucheron2016segmentation}, wherein the images are corrected for limb brightening following the method outlined in \cite{verbeeck2014}. An initial seed is then generated by selecting all on-disk pixels with an intensity $\leq\alpha\times QS$ where $QS$ is the mean intensity of the quiet Sun, and the seeding parameter ($\alpha$) is defined as $\alpha=0.3$. From there ACWE was performed on the on-disk region using the length constraint $\mu=0$, and the ratio of foreground to background homogeneity parameters $\lambda_i/\lambda_o=50$.

The compression process was evaluated using four 193~{\AA} Solar EUV images with record times (as expressed by the \verb.T_REC. keyword) 2010-07-25 T12:00:02Z, 2010-08-21 T22:00:02Z, 2010-09-18 T00:00:02Z, and 2013-02-21 T23:00:01Z. In order to prepare the images for the compression process, the original Level 1 EUV image (at their native spatial resolution of $4096\times4096$ pixels) were clipped to the intensity range of $[20,2500]$. Once clipped, a $\log_{10}$ transform was applied to the intensity levels within images. The resulting intensities where then mapped to 255 discrete levels before performing the compression using the proposed network (with both WNLAM and WCBAM attention). For this process eight models were developed using the hyper-parameters $\lambda=\{0.0005, 0.0035, 0.007, 0.009, 0.011, 0.0125, 0.019, 0.025\}$. Once a compressed image for each EUV input was generated from each model, the images were then restored by reversing the intensity mapping and reversing the $\log_{10}$ transform prior to performing ACWE.

An example of the effects of the proposed compression scheme on the final CH segmentation is presented in Fig. \ref{fig:ACWEneuralExample}. In this figure the output of the compressed images are organized by descending PSNR of the compressed image, and titled with PSNR and bit-rate of the compressed image. Besides the first two images in Fig. \ref{fig:ACWEneuralExample}, which are the original solar EUV image and the CH segmentation generated from the original image, each image is a comparison between the two segmentations (original and compressed) wherein purple regions were only identified as CHs in the original segmentation, yellow regions were identified as belonging to a CH only in the compressed image segmentation, green regions were identified as CHs in both segmentations, and blue regions were not identified as CHs in either segmentation. Within this image set, and the remaining cases tested, the discrepancies between segmentations are generally limited to small-scale structures, usually along the boundary of CH regions. This suggests that the proposed compression scheme is able to preserve the overall structure (and intensity) of coronal hole regions within the solar EUV image. 

Across the four images, the effects of compression were evaluated by computing the DICE coefficient, defined as 
\begin{equation}
    DSC = \frac{2|S_1\cap S_2|}{|S_1|+|S_2|},
\end{equation}
between the CH segmentation generated by ACWE from the original EUV image ($S_1$), and the segmentation generated from the compressed image ($S_2$), where $|\cdot|$ denotes cardinality and $\cap$ denotes intersection. These results, which are shown as a function of bit rate of the compressed image in Fig. \ref{fig:ACWEneuralDice}, corroborate the observations seen in Fig. \ref{fig:ACWEneuralExample} by showing high similarity between segmentations across all bit rates.

It should be noted that applying a log transformation to the intensities within an image increases the number of output intensity levels used to represent low intensities while decreasing the number of output levels used to represent high intensities% \cite{DIPbook}
. For this reason, more of the 255 discrete intensity levels were allocated to preserving fine detail at the low intensity range of the image, which, in turn, improved the quality of the ACWE segmentation \cite{grajeda2023}. 

To help disentangle the effects of this advantage, this same prepossessing was applied to the same EUV images before compressing the images using JPEG compression, then reversing the process in the same manner. The DICE coefficient (again, compared to the segmentation of the original EUV image) as a function of the bit-rate of the compressed image for the JPEG compression scheme is presented in Fig. \ref{fig:ACWEjpegDice}. It should be noted that the JPEG compression scheme begins to show signs of degradation in image features that negatively impact CH segmentation at compression rates of $\sim0.12$ bits per pixel, and cannot produce images with a compression rate $<0.1$ bits per pixel.  One the other hand, the neural compression scheme proposed here continues to perform well beyond this threshold, suggesting that the neural compression scheme is able to better preserve the features that are relevant to this application.  

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{figs/ACWE/neuralACWEresize_param1.DICE.pdf}
    \caption{Effects of proposed compression scheme on CH detection via ACWE, expressed as DICE coefficient as a function of bit-rate.}
    \label{fig:ACWEneuralDice}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{figs/ACWE/jpegACWEresize_param1.DICE.pdf}
    \caption{Effects of JPEG compression scheme on CH detection via ACWE, expressed as DICE coefficient as a function of bit-rate.}
    \label{fig:ACWEjpegDice}
\end{figure}
